Optimization for Amortized Inverse Problems

Incorporating a deep generative model as the prior distribution in inverse problems has established substantial success in reconstructing images from corrupted observations. Notwithstanding, the existing optimization approaches use gradient descent largely without adapting to the non-convex nature of the problem and can be sensitive to initial values, impeding further performance improvement. In this paper, we propose an efficient amortized optimization scheme for inverse problems with a deep generative prior. Specifically, the optimization task with high degrees of difficulty is decomposed into optimizing a sequence of much easier ones. We provide a theoretical guarantee of the proposed algorithm and empirically validate it on different inverse problems. As a result, our approach outperforms baseline methods qualitatively and quantitatively by a large margin.

==> subfiles/old_intro.tex <==
--------------Previous version by Lei, Qi------------

Inverse problems using generative models aim to reconstruct an image/signal $\xv$ via a noisy or lossy observation  $$ \yv = f(\xv) + \ev,$$
{with the assumption that } $\xv$ comes from a generative model $G$, i.e., $\xv=G(\zv)$ for some latent code $\zv$~\citep{bora2017compressed}.  $f(\cdot)$ is a known forward operator and $\ev$ represents noise.  The problem is reduced to  denoising  when $f(\xv) = \xv$ is the identity map, and is reduced to a compressed sensing~\citep{candes2006stable,donoho2006compressed}, inpainting~\citep{vitoria2018semantic}, or super-resolution problem~\citep{menon2020pulse} when $f(\xv) =\Amat \xv$ and $\Amat$ maps $\xv$ to a lower dimensional space. As an under-determined problem, inverse problems require some proper assumptions on the prior of the image. Instead of more classical assumptions like sparsity or other geometric properties on $\xv$~\citep{danielyan2011bm3d,yu2011solving}, deep generative prior has recently become the workhorse of inverse problems \citep{bora2017compressed,asim2020blind}. Existing works on solving inverse problems  often design the objective by
\begin{align}
\label{eqn:reconstruction}
    \hat\zv = \argmin\nolimits_{\zv} \mathcal{L}_{\text{recon}}(G(\zv), \yv) + \lambda \mathcal{L}_{\text{reg}}(\zv),
\end{align}
 where $\mathcal{L}_\text{recon}$  is a reconstruction error between the observation $\yv$ and a recovered image $G(\zv)$~\citep{bora2017compressed,ulyanov2018deep}, and $\mathcal{L}_{\text{reg}}(\zv)$ multiplied by hyperparameter $\lambda$ regularizes  $\zv$ via incorporating prior information of its latent  distribution. The loss function is subject to different noise models~\citep{van2018compressed,asim2020invertible,whang21solve}.  The image is reconstructed as $\hat \xv = G(\hat \zv)$. 


In execution, however, the challenges are two-fold. The success of this model fundamentally relies on a correct choice of the hyperparameter $\lambda$ and an effective optimization algorithm that can find the global minimum of \eqref{eqn:reconstruction}. 
However, the non-convex nature of inverse problems makes optimization algorithms unprincipled and non-robust (to choices like initialization). 
\qilei{add discussion with the NP-hardness. brief discussion about the difficulty when it comes to overdetermined problem  -- current analysis in optimization is usually regarding to overparameterized NNs..   the optimization for inverse problem is by design more challenging}

%\qilei{also emphasize the importance of efficiency. not user-friendly if the performance is not real-time. }

We thus raise the following  question:

{\em \textbf{Question.} Can we design a more principled optimization scheme that makes use of the structure of the objective and even bears theoretical guarantees? }

In general, reconstructing the latent code from the observations of a deep neural network is NP-hard \citep{lei2019inverting}. Therefore we must utilize some special structure of the problem to resolve it efficiently.  


In this paper, we resolve the above question by introducing \qilei{to add}


\begin{itemize}
\item We propose an amortized optimization scheme that incrementally optimizes the solution on a sequence of $\lambda$ that gradually increase from 0 to our desired value. 
% \vspace{-2mm}
\item We provide theoretical guarantees on finding the global minimum of our algorithm for denoising tasks, under some natural assumptions. 
% \vspace{-2mm}
\item We propsoe an automatic entropy-preserving hyperparameter tuning scheme without any human evaluation.
% \vspace{-2mm}
\item We bring together the two schemes and propose {\notion},
an end-to-end inverse problem solver
under the maximum a posterior (MAP) framework.%, by combining a cascade optimization algorithm and an entropy-preserving hyperparameter tuning.
% \vspace{-2mm}
\end{itemize}
%We propose an automated hyper-parameter tuning  {scheme}  for inverse problems  through a formulation of a model-based bilevel optimization objective. We empirically  {demonstrate} the performance on different tasks of inverse problems  and show  a significant convenience and efficiency of our approach compared to hand-tuned grid search. 

    
Our paper proceeds as follows. We discuss the related works in Section~\ref{sec:literature}, including inverse problems with deep generative priors and hyperparameter tuning in general machine learning. We propose our core algorithms in Section~\ref{sec:method} and provide theoretical guarantees in Section~\ref{sec:map-fix-beta-thm}. In Section~\ref{sec:experiment}, we empirically validate the performance of our algorithm, which outperforms commonly used approaches. Section~\ref{sec:conclustion} concludes the paper.
Supplementary algorithms and proofs are deferred to the appendix.






